Multi-Petawatt Physics Prioritization (MP3) Workshop Report

This Multi-Petawatt Physics Prioritization (MP3) Workshop Report captures the outcomes from a community-initiated workshop held April 20-22, 2022 at Sorbonne University in Paris, France. The MP3 workshop aimed at developing science questions to guide research and future experiments in four areas identified by corresponding MP3 working groups: high-field physics and quantum electrodynamics (HFP/QED), laboratory astrophysics and planetary physics (LAPP), laser-driven nuclear physics (LDNP), and particle acceleration and advanced light sources (PAALS).

==> MP3-White_papers_full.tex <==

\includepdf[pages={-}]{figures/Blank_Page.pdf}

\section{White Papers}
%\addcontentsline{toc}{part}{White Papers}
\label{sec-WP}

This appendix contains a list of the white paper author(s) and titles that were received for the MP3 workshop. Listed in the order they were received. The list is linked to the full text of each white paper as they were submitted.


\begin{enumerate}
   
\item \hyperlink{link_002}{Markus Roth, Marc Zimmer, Stefan Scheuren, Christian R\"{o}del, \textit{Laser Neutron Production entering the Spallation Mode}}
\label{MP3_002}

\item \hyperlink{link_003}{J.P. Palastro, A. Arefiev, J. Bromage, M. Campbell, A. Di Piazza, M. Formanek, P. Franke, D.H. Froula, B. Malaca, W. Mori, J. Pierce, D. Ramsey, J.L. Shaw, T.T. Simpson, J. Vieira, M. Vranic, K. Weichman, J. Zuegel, \textit{Novel Plasma Physics Regimes enabled by Spatiotemporally Shaped Laser Pulses}}
\label{MP3_003}

\item \hyperlink{link_004}{Xing-Long Zhu, and Zheng-Ming Sheng, \textit{Ultra-brilliant GeV gamma-ray emission with multi-petawatt lasers}}
\label{MP3_004}

\item \hyperlink{link_005}{Henry P. Freund, \textit{Advanced Light Sources with Polarization Control Based upon Laser-Based Accelerators}}
\label{MP3_005}

\item \hyperlink{link_006}{Yasuhiko Sentoku, Natsumi Iwata, Mamiko Nishiuchi, Alexey Arefiev, \textit{Dynamics of multi-petawatt laser driven high Z radiative plasmas}}
\label{MP3_006}

\item \hyperlink{link_007}{D. Stutman, M.P. Valdivia, D. Kumar, M. O. Cernaianu, D. Doria, P. Ghenuche, N. Safca, \textit{Phase-based X and gamma ray diagnostics for multi-Petawatt laser research}}
\label{MP3_007}

\item \hyperlink{link_008}{Hans Rinderknecht, A. Arefiev, T. Toncian, M. Wei, T. Wang, G. Bruhaug, A. Laso Garcia, K. Weichman, J. Palastro, D. Doria, K. Spohr, M. Cernaianu, P. Ghenuche, J. Williams, A. Haid, T. Ditmire, H. Quevedo, and Dan Stutman, \textit{Relativistically transparent magnetic filaments: a platform for high-field science and efficient gamma-ray sources}}
\label{MP3_008}

\item \hyperlink{link_009}{Kathleen Weichman, M. Murakami, J.J. Honrubia, S.V. Bulanov, J.K. Koga, M.A.H. Zosa, A.V. Arefiev, and J. Palastro, \textit{Microcavity implosions for the generation of extreme electric fields and ultrahigh magnetic fields}}
\label{MP3_009}

\item \hyperlink{link_010}{Oleg B.\ Shiryaev, Michael Yu.\ Romanovsky, and Vladimir V.\ Bukin, \textit{Vacuum post-acceleration of relativistic electrons by combinations of THz electromagnetic pulses and constant magnetic fields}}
\label{MP3_010}

\item \hyperlink{link_011}{Stephane Branly, Franck Falcoz, Catalin Neacsu, Kaikai Zhang and Pierre-Mary Paul, \textit{Status and future of high energy high average power lasers}}
\label{MP3_011}

\item \hyperlink{link_012}{James K. Koga, Masaki Kando, Sergei V. Bulanov, Timur Zh. Esirkepov, Alexander S. Pirozhkov, Petr Valenta, Tae Moon Jeong, Georg Korn, Stepan S. Bulanov, \textit{Relativistic Flying Mirrors for Fundamental Science and Applications}}
\label{MP3_012}

\item \hyperlink{link_013}{T. Heinzl, A. Ilderton, and B. King, \textit{Laser-Matter Interactions at the Intensity Frontier}}
\label{MP3_013}

\item \hyperlink{link_014}{Zsolt L\'{e}cz1, and Alexander Andreev, \textit{Positron detection for plasma and field diagnostics in high-power laser-solid interactions}}
\label{MP3_014}

\item \hyperlink{link_015}{Bal\v{s}a Terzi\'{c}, and Geoffrey Krafft, \textit{Improving Performance of Inverse Compton Sources in High-Field Regime via Laser Chirping}}
\label{MP3_015}

\item \hyperlink{link_016}{D. Seipt, M. Zepf, and S. G. Rykovanov, \textit{Advanced Concepts for Monoenergetic $\gamma$-Ray Generation using Nonlinear Compton Scattering}}
\label{MP3_016}

\item \hyperlink{link_017}{Shuta J. Tanaka, Keita Seto, Yasuhiro Kuramitsu, Yuji Fukuda, and Youichi Sakawa, \textit{Experimental observation of induced Compton scattering}}
\label{MP3_017}

\item \hyperlink{link_018}{Felix Karbstein, Holger Gies, Elena A. Mosman, Gerhard
G. Paulus, Kai S. Schulze, and Thomas St\"{o}hlker, \textit{Co-location of a multi-petawatt laser with an x-ray free electron laser}}% (HFP/QED)}
\label{MP3_018}

\item \hyperlink{link_019}{Deepak Kumar, Chris Armstrong, Florian Condamine, Thomas Cowan, Alejandro Laso Garcia, Tae Moon Jeong, Ond\v{r}ej Klimo, Paul McKenna, Alexander Pirozhkov, Sushil Singh, Dan Stutman, Vladimir Tikhonchuk, Roberto Versaci, June Wicks, \textit{High energy X-ray diagnostics for interaction of a high repetition rate multi-petawatt laser with solid targets}}
\label{MP3_019}

\item \hyperlink{link_020}{Holger Gies, Felix Karbstein, J\"{o}rg Schreiber, and Matt Zepf, \textit{Quantum vacuum signatures in laser pulse collisions}}
\label{MP3_020}

\item \hyperlink{link_021}{Hiroshi Sawada, \textit{Relativistic Electron Isochoric Heating with Petawatt Femtosecond Lasers for Creation of Warm Dense Matter}}
\label{MP3_021}

\item \hyperlink{link_022}{Peter V. Heuer, Hans G. Rinderknecht, Derek B. Schaeffer, Scott Feister, \textit{The Role of High Repetition Rate Experiments in Advancing HEDP Science}}
\label{MP3_022}

\item \hyperlink{link_023}{Karl Krushelnick, \textit{Laser wakefield acceleration with Multi Petawatt lasers}}
\label{MP3_023}

\item \hyperlink{link_024}{Matteo Tamburini, Antonino Di Piazza, Christoph H. Keitel, \textit{The quest for precision measurements of strong-field QED effects}}
\label{MP3_024}

\item \hyperlink{link_025}{Yan-Fei Li, Wei-Min Wang, Yu-Tong Li, \textit{The interaction of a multi-petawatt laser pulse with an ultrarelativistic electron beam could be utilized to produce polarized positron-beam source or conduct confirmatory experiments on QED theory}}
\label{MP3_025}

\item \hyperlink{link_026}{Bruce A. Remington, Hui Chen, \textit{Relativistic astrophysical jets from accreting massive black holes in galactic centers}}
\label{MP3_026}

\item \hyperlink{link_027}{Hui Chen, Frederico Fiuza, and Bruce Remington, \textit{Laser produced relativistic pair plasmas in the laboratory}}
\label{MP3_027}

\item \hyperlink{link_028}{Stephanie Hansen, and Brent Jones, \textit{MP3 Opportunities for Benchmark-quality Lab-Astro Experiments}}
\label{MP3_028}

\item \hyperlink{link_029}{Reinhard Alkofer, Matthias Diez, and Christian Kohlf\"{u}rst \textit{What are the time-scales of particle formation in the Schwinger effect?}}
\label{MP3_029}

\item \hyperlink{link_030}{Ronnie Shepherd, Mark Sherlock, Max Tabak, Steve Libby, Yuan Shi, Nathaniel Roth, Hui Chen, Howard Scott, \textit{Soft X-ray emission spectroscopy to search for Unruh radiation}}
\label{MP3_030}

\item \hyperlink{link_031}{Wendell T Hill, III, Andrew Longman, Calvin Z He, Smrithan Ravichandran, José Antonio Pérez-Hernández, Jon I Apiñaniz, Roberto Lera, Luis Roso, and Robert Fedosejevs, \textit{Direct Measure of Quantum Vacuum Properties}}
\label{MP3_031}

\item \hyperlink{link_032}{Luis Roso, Andrew Longman, Calvin Z He, Smrithan Ravichandran, Jose Antonio Pérez-Hernández, Jon I Apiñaniz, Roberto Lera, Robert Fedosejevs, and Wendell T Hill, III \textit{Radiation from the electron-positron virtual pairs accompanying laser driven electrons.}}
\label{MP3_032}

\item \hyperlink{link_033}{Robert Fedosejevs, Andrew Longman, Calvin Z He, Smrithan Ravichandran, Jose Antonio Pérez-Hernández, Jon I Apiñaniz, Roberto Lera, Luis Roso, and Wendell T Hill, III, \textit{In situ intensity gauge adapted for extremely-high intensities}}
\label{MP3_033}

\item \hyperlink{link_034}{Ondrej Klimo, Stefan Weber, \textit{Controlled $\gamma$-ray secondary source}}
\label{MP3_034}

\item \hyperlink{link_035}{Marcelo Ciappina, Stefan Weber, \textit{Atomic high-field diagnostic using multiple sequential ionization}}
\label{MP3_035}

\item \hyperlink{link_036}{Caterina Riconda, Stefan Weber, \textit{Plasma Amplification for High-Power Lasers}}
\label{MP3_036}

\item \hyperlink{link_037}{N. Iwata, Y. Sentoku, A. J. Kemp, and S. C. Wilks, \textit{Stochastic laser-plasma interaction with kJ-class petawatt laser light}}
\label{MP3_037}

\item \hyperlink{link_038}{Timur Zh. Esirkepov, Akito Sagisaka, Koichi Ogura, Hiromitsu Kiriyama, James K. Koga, Masaki Kando, Danila R. Khikhluha, Ilia P. Tsygvintsev, Chris D. Armstrong, Deepak Kumar, Stepan S. Bulanov, Georg Korn, Sergei V. Bulanov, Alexander S. Pirozhkov, \textit{Experimental Access to Laser-Driven Gamma Flare}}
\label{MP3_038}

\item \hyperlink{link_039}{Calin Ioan Hojbota, Mohammad Rezaei-Pandari, Mohammad Mirzaie, Vishwa Bandhu Pathak, Doyeon Kim, Jeongho Jeon, Kiyong Kim, Chang Hee Nam, \textit{Muon production for the detection of high-energy photons from laser-electron collisions}}
\label{MP3_039}

\item \hyperlink{link_040}{G. Sarri, M. Streeter, L. Calvin, N. Cavanagh, \textit{High-energy and high-quality positron beams from a laser wake-field accelerator}}
\label{MP3_040}

\item \hyperlink{link_041}{G. Sarri, M. Streeter, L. Calvin, N. Cavanagh, K. Fleck \textit{High-field quantum electrodynamics in the field of an intense laser}}
\label{MP3_041}

\item \hyperlink{link_042}{Sergei V. Bulanov, Prokopis Hadjisolomou, Gabriele Grittani, Tae Moon Jeong, Georg Korn, Danila R. Khikhlukha, Pavel V. Sasorov, Petr Valenta, Kirill V. Lezhnin, Ilia P. Tsygvintsev, Vladimir A. Gasilov, Timur Zh. Esirkepov, Alexander S. Pirozhkov, James K. Koga, Masaki Kando, Tetsuya Kawachi, \textit{High Power Gamma Flashes Generated in Multi-Petawatt Laser-Matter Interaction for Fundamental Science and Applications}}
\label{MP3_042}

\item \hyperlink{link_043}{Thomas G. White, Matthew Oliver, and Tilo D\"{o}ppner, \textit{Measurements of Transport Properties in Warm Dense Matter with Multi-Petawatt Lasers}}
\label{MP3_043}

\item \hyperlink{link_044}{K. Matsuo, M. Bailly-Grandvaux, S. Bolanos, D. Kawahito, C. McGuffey,
M. Dozières, J. Peebles, J. R. Davies, M.S. Wei, W. Theobald, P.-A. Gourdain, J. Honrubia, J.J. Santos, and F.N. Beg, \textit{Energy deposition in magnetized dense plasma by laser-driven relativistic electrons}}
\label{MP3_044}

\item \hyperlink{link_045}{Matthias Fuchs \textit{Next-generation Lightsources and Applications}}
\label{MP3_045}

\item \hyperlink{link_046}{Lili Manzo, Matthew Edwards, Yuan Shi, \textit{Enhancing hot electron generation via magnetized laser absorption}}
\label{MP3_046}

\item \hyperlink{link_047}{J. Kim, D. Mariscal, B. Djordjevic, \textit{Efficient laser-driven ion acceleration using temporally shaped high-intensity pulses}}
\label{MP3_047}

\item \hyperlink{link_048}{C. B. Schroeder, C. Benedetti, E. Esarey, C. G. R. Geddes, J. van Tilborg, \textit{Laser wakefield acceleration using multi-PW lasers}}
\label{MP3_048}

\item \hyperlink{link_049}{F\'{e}licie Albert \textit{X-ray light sources from laser plasma acceleration and their applications}}
\label{MP3_049}

\item \hyperlink{link_050}{Andreas Kemp, S.C.Wilks, G.Grim, E.Hartouni, S.Kerr, G.Cochran \textit{Development of a new laser-based platform capable of measuring nuclear reaction rates in hot plasmas}}
\label{MP3_050}

\item \hyperlink{link_051}{Amina E. Hussein, \textit{Multi-petawatt electron acceleration and strong magnetic field generation}}
\label{MP3_051}

\item \hyperlink{link_052}{G. Gregori, S. Sarkar, R. Bingham, C. H.-T. Wang, \textit{Going Beyond the Standard Model with High Power Lasers}}
\label{MP3_052}

\item \hyperlink{link_053}{Pierre Gourdain, and Georg Hoffstaetter, \textit{Using inverse Compton scattering from a short pulse laser to measure the properties of warm dense matter produced by pulsed-power drivers}}
\label{MP3_053}

\item \hyperlink{link_054}{P. Neumayer, V. Bagnoud, \textit{Research at the high-energy short-pulse laser system PHELIX user facility}}
\label{MP3_054}

\item \hyperlink{link_055}{Keita Seto, Jian Fuh Ong, Yoshihide Nakamiya, Mihai Cuciuc, Stefan Ataman, Cesim
Dumlu, Madalin Rosu, Ovidiu Tesileanu, Takahisa Jitsuno, and Kazuo A. Tanaka, \textit{Radiation reaction experiment with 60 PW laser pulse and 10 GeV electron bunch}}
\label{MP3_055}

\item \hyperlink{link_056}{Bruce A. Remington and Hui Chen, \textit{High power laser experiments probing plasma nuclear science}}
\label{MP3_056}

\item \hyperlink{link_057}{Alexandru Măgureanu, Viorel Nastasa, Deepak Sangwan, Bogdan Diaconescu, Dan G. Ghiţă, Marius Gugiu, Theodor Asavei, Zhehui Wang, Cătălin M. Ticoş, \textit{Machine Learning for 3D Reconstruction of High Density Laser-Plasma}}
\label{MP3_057}

\item \hyperlink{link_058}{Andrei Tudor Patrascu, \textit{Unruh Radiation Detection}}
\label{MP3_058}

\item \hyperlink{link_059}{K. M. Spohr, D. Doria, K. A. Tanaka, G. Bruhaug, C. Forrest, and H. Rinderknecht, et al., \textit{Nuclear physics research in laser induced plasma with a multi-petawatt laser system: production and decay studies of cosmogenic 26Al}}
\label{MP3_059}

\item \hyperlink{link_060}{K. M. Spohr, D. Doria, K. A. Tanaka, M. O. Cernaianu, D. O’Donnell, V. Nastasa, P. Ghenuche, P. A. Söderström, G. Bruhaug, C. Forrest, and H. Rinderknecht, \textit{Laser-driven population and release of the 2.4 MeV isomer in 93Mo, towards a `Nuclear Battery'}}
\label{MP3_060}

\item \hyperlink{link_061}{Cesim K. Dumlu, Keita Seto, Stefan Ataman, Jian-Fuh Ong, Ovidiu Tesileanu and Kazuo A. Tanaka, \textit{A Proposal for the Observation of Pair Production in Intense Field Regime}}
\label{MP3_061}

\item \hyperlink{link_062}{M. Vranic, T. Grismayer, A. AreBiev, H. Chen, S. Corde, R. A. Fonseca, M. Grech, C. Joshi, A. G. R. Thomas, B. Martinez, S. Meuren, W. B. Mori, C. Riconda, C. Ridgers, D. Seipt, L. O. Silva, T. Silva, J. Vieira, L. Willingale, \textit{Positron creation and acceleration with multi-petawatt lasers}}
\label{MP3_062}

\item \hyperlink{link_063}{Stefan Ataman, Keita Seto, Cesim Dumlu, Jian-Fuh Ong, Andrei Berceanu, Ovidiu Tesileanu, Kazuo A. Tanaka, \textit{MP3 all-optical vacuum birefringence experiment proposal}}
\label{MP3_063}

\item \hyperlink{link_064}{Domenico Doria, A. Arefiev, M. O. Cernaianu, P. Ghenuche, K. Spohr, K. A. Tanaka, \textit{Laser driven-acceleration of ion and energy scaling modification by competitive processes.}}
\label{MP3_064}

\item \hyperlink{link_065}{Edison Liang, \textit{High-Energy Astrophysics Experiments Based on Ultra-intense Lasers Irradiating Solid Targets}}
\label{MP3_065}

\item \hyperlink{link_066}{Sergei V. Bulanov, Yan Gun Gu, \textit{Magnetic field annihilation and charged particle acceleration in ultra-relativistic laser plasmas}}
\label{MP3_066}

\item \hyperlink{link_067}{P. Ghenuche, M. O. Cernaianu, D. Stutman, F. Negoita, D.L. Balabanski, A. V. Arefiev, D. Schumacher, and, D. Doria, \textit{Enhanced laser-plasma experiments with helical laser beams}}
\label{MP3_067}

\item \hyperlink{link_068}{Edmond Turcu, \textit{Electron-Positron Pair Production Interaction Chambers with Counter-propagating, Colliding multi-PW Laser Pulses}}
\label{MP3_068}

\item \hyperlink{link_069}{M. Grech, L. Lancia, I. A. Andriyash, P. Audebert, A. Beck, S. Corde, X. Davoine, M. Frotin, A. Grassi, L. Gremillet, S. Le Pape, M. Lobet, A. Leblanc, F. Mathieu, F. Massimo, A. Mercuri-Baron, D. Papadopoulos, F. P\'{e}rez, J. Prudent, C. Riconda, L. Romagnani, A. Specka, C. Thaury, K. Ta Phuoc, T. Vinci, \textit{Investigating strong-field QED processes in laser-electron beam collisions at Apollon}}
\label{MP3_069}

\item \hyperlink{link_070}{C. A. J. Palmer, B. Reville, A. R. Bell, A. F. A. Bott, H. Chen, G. Gregori, D. Lamb, C. K. Li, J. Matthews, J. Meinecke, H-S.Park, R. Petrasso, S. Sarkar, A. Schekochihin, L. Silva, A. Robinson, P. Tzeferacos, and M. Vranic, \textit{Exploring cosmic-ray physics with high-energy, high-intensity lasers}}
\label{MP3_070}

\item \hyperlink{link_071}{Jian-Xing Li, Yue-Yue Chen, Yan-Fei Li, Karen Z. Hatsagortsyan, Christoph H. Keitel, \textit{Generation of polarized high-energy lepton and photon beams}}
\label{MP3_071}

\item \hyperlink{link_072}{Sergei V. Bulanov, Gabriele Grittani, Tae Moon Jeong, Martin Jirka, Georg Korn, Pavel V. Sasorov, Timur Zh. Esirkepov, James K. Koga, Stepan S. Bulanov, Francesco Pegoraro, \textit{Nonlinear Electromagnetic Waves in Quantum Vacuum}}
\label{MP3_072}

\item \hyperlink{link_073}{Matteo Tamburini, Brian Reville, Jim Hinton, Christoph H. Keitel, \textit{Laboratory gamma-electron-positron plasma – a new frontier in strong-field QED and relativistic laboratory astrophysics}}
\label{MP3_073}

\item \hyperlink{link_074}{Sergei V. Bulanov, Timur Z. Esirkepov, Stepan S. Bulanov, \textit{Compact Hadron Collider with the Ion Accelerator Using the Laser Radiation Pressure}}
\label{MP3_074}

\item \hyperlink{link_075}{J. Fuchs, W. Yao, V. Horny, K. Burdonov, C. Ruyer, L. Gremillet. X. Davoine, E. d’Humières, X. Ribeyre, S.N. Chen, D. Schaeffer, W. Fox, P. Heuer, \textit{Towards investigating astrophysically relevant fast collisionless shocks}}
\label{MP3_075}

\item \hyperlink{link_076}{Sebastian Meuren, David A. Reis, Roger Blandford, Phil H. Bucksbaum, Nathaniel
J. Fisch, Frederico Fiuza, Elias Gerstmayr, Siegfried Glenzer, Mark J. Hogan, Claudio
Pellegrini, Michael E. Peskin, Kenan Qu, Glen White, and Vitaly Yakimenko, \textit{Research Opportunities Enabled by Co-locating Multi-Petawatt Lasers with Dense Ultra-Relativistic Electron Beams}}
\label{MP3_076}

\item \hyperlink{link_077}{Vishwa Bandhu Pathak, Calin Ioan Hojbota, Mohammad Mirzaie, and Chang Hee Nam, \textit{Electron acceleration beyond the single-stage laser wakefield acceleration}}
\label{MP3_077}

\item \hyperlink{link_078}{J. Fuchs, V. Horny, K. Burdonov, V. Lelasseux, W. Yao, L. Gremillet. X. Davoine, E. d’Humi\`{e}res, X. Rib\`{e}re, S.N. Chen, F. Negoita, P-A S\"{o}derstr\"{o}m, I. Pomerantz, \textit{Opening the experimental investigation of heavy elements nucleosynthesis through extreme brightness neutron beams generated by multi-PetaWatt-class lasers}}
\label{MP3_078}

\item \hyperlink{link_079}{P. Zhang, S. S. Bulanov, D. Seipt, A. V. Arefiev, and A. G. R. Thomas, \textit{Relativistic Plasma Physics in Supercritical Fields}}
\label{MP3_079}

\item \hyperlink{link_080}{D. Seipt, C. P. Ridgers, M. Vranic, T. Grismayer, and A. G. R. Thomas, \textit{Spin and Polarization in High-Intensity Laser-Matter Interactions}}
\label{MP3_080}

\item \hyperlink{link_081}{Chris Fryer, Shane Coffing, Suzannah Wood, Chris Fontes, Todd Urbatsch, \textit{Understanding Transients: Needs from the Laboratory Astrophysics Community}}
\label{MP3_081}

%\item \textit{Self-Focussing of an Intense X-Ray Beam in Vacuum}
%\label{MP3_082}

\item \hyperlink{link_083}{Brandon K. Russell, Marija Vranic, Paul T. Campbell, Kevin M. Schoeffler, Alexander G. R. Thomas, Dmitri Uzdensky, and Louise Willingale, \textit{Electron-only radiation dominated magnetic reconnection}}
\label{MP3_083}

%\item Gilbert Collins, Tom Duffy, Danae Polsin, Scott Wilks, Gianluca Gregori, Eva Zurek, \textit{Multi-Petawatt Laser Systems to Interrogate Matter at Atomic Pressures}
%\label{MP3_084}
% This paper is the same as MP3_091

\item \hyperlink{link_085}{J. Fuchs, W. Yao, V. Horny, K. Burdonov, L. Gremillet, X. Davoine, E. d’Humi\`{e}res, X. Rib\`{e}yre, S.N. Chen, \textit{Enhanced laser coupling, matter heating, and particle acceleration by multiplexing PetaWatt-class lasers}}
\label{MP3_085}   
   
\item \hyperlink{link_086}{B. Manuel Hegelich, Lance Labun, Ou Zhang, \textit{Performance metrics for laser-electron colliders to aid design and discovery}}
\label{MP3_086}

\item \hyperlink{link_087}{James P. Edwards, Misha A. Lopez-Lopez, Christian Schubert, \textit{Photon-photon scattering in a plane-wave background}}
\label{MP3_087}
   
\item \hyperlink{link_088}{G. Bruhaug, H. G. Rinderknecht, J.R. Rygg, G. Collins, Y. E, K. Garriga, X.C. Zhang, \textit{Extreme THz Pulse Generation and Interaction with Matter}}
\label{MP3_088}

\item \hyperlink{link_089}{M. Lyutikov, \textit{Astrophysical analogues of laser-plasma interaction}}
\label{MP3_089}

\item \hyperlink{link_090}{M. C. Marshall, D. N. Polsin, G. Bruhaug, G. W. Collins, and J. R. Rygg, \textit{Ultrafast phase transformation studies in planetary materials to terapascal pressures using x-ray and electron diffraction}}
\label{MP3_090}

\item \hyperlink{link_091}{Gilbert Collins, Tom Duffy, Danae Polsin, Scott Wilks, Gianluca Gregori, Eva Zurek, \textit{Multi-Petawatt Laser Systems to Interrogate Matter at Atomic Pressures}}
\label{MP3_091}

\item \hyperlink{link_092}{Henry Freund, \textit{Discussion of XFELs \& Laser-Driven FELs Petawatt Laser Initiative}}
\label{MP3_092}

\item \hyperlink{link_093}{Ion Cristian Edmond Turcu, \textit{Colliding Relativistic Light-Sails accelerated by Multi-PW lasers}}
\label{MP3_093}

\item \hyperlink{link_094}{Klaus Steiniger, Alexander Debus, and Ulrich Schramm, \textit{Petawatt Class Lasers for Realizing Optical Free-Electron Lasers with Traveling-Wave Thomson-Scattering}}
\label{MP3_094}

\item \hyperlink{link_095}{Alexander Debus, Klaus Steiniger, Ulrich Schramm, \textit{Scaling Laser-Plasma Electron Accelerators to 100GeV-scale Energies using TWEAC and Multi-Petawatt Lasers}}
\label{MP3_095}
   
\end{enumerate}

% To reference a white paper in the text, you would refer to White Paper \ref{WP1}, for example.



%Full White paper attachments

\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_002}{\includepdf[pages={-}]{WP_pdfs/MP3_002.pdf}}
\hypertarget{link_003}{\includepdf[pages={-}]{WP_pdfs/MP3_003.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_004}{\includepdf[pages={-}]{WP_pdfs/MP3_004.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_005}{\includepdf[pages={-}]{WP_pdfs/MP3_005.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_006}{\includepdf[pages={-}]{WP_pdfs/MP3_006.pdf}}
\hypertarget{link_007}{\includepdf[pages={-}]{WP_pdfs/MP3_007.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_008}{\includepdf[pages={-}]{WP_pdfs/MP3_008.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_009}{\includepdf[pages={-}]{WP_pdfs/MP3_009.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_010}{\includepdf[pages={-}]{WP_pdfs/MP3_010.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_011}{\includepdf[pages={-}]{WP_pdfs/MP3_011.pdf}}
\hypertarget{link_012}{\includepdf[pages={-}]{WP_pdfs/MP3_012.pdf}}
\hypertarget{link_013}{\includepdf[pages={-}]{WP_pdfs/MP3_013.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_014}{\includepdf[pages={-}]{WP_pdfs/MP3_014.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_015}{\includepdf[pages={-}]{WP_pdfs/MP3_015.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_016}{\includepdf[pages={-}]{WP_pdfs/MP3_016.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_017}{\includepdf[pages={-}]{WP_pdfs/MP3_017.pdf}}
\hypertarget{link_018}{\includepdf[pages={-}]{WP_pdfs/MP3_018.pdf}}
\hypertarget{link_019}{\includepdf[pages={-}]{WP_pdfs/MP3_019.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_020}{\includepdf[pages={-}]{WP_pdfs/MP3_020.pdf}}
\hypertarget{link_021}{\includepdf[pages={-}]{WP_pdfs/MP3_021.pdf}}
\hypertarget{link_022}{\includepdf[pages={-}]{WP_pdfs/MP3_022.pdf}}
\hypertarget{link_023}{\includepdf[pages={-}]{WP_pdfs/MP3_023.pdf}}
\hypertarget{link_024}{\includepdf[pages={-}]{WP_pdfs/MP3_024.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_025}{\includepdf[pages={-}]{WP_pdfs/MP3_025.pdf}}
\hypertarget{link_026}{\includepdf[pages={-}]{WP_pdfs/MP3_026.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_027}{\includepdf[pages={-}]{WP_pdfs/MP3_027.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_028}{\includepdf[pages={-}]{WP_pdfs/MP3_028.pdf}}
\hypertarget{link_029}{\includepdf[pages={-}]{WP_pdfs/MP3_029.pdf}}
\hypertarget{link_030}{\includepdf[pages={-}]{WP_pdfs/MP3_030.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_031}{\includepdf[pages={-}]{WP_pdfs/MP3_031.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_032}{\includepdf[pages={-}]{WP_pdfs/MP3_032.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_033}{\includepdf[pages={-}]{WP_pdfs/MP3_033.pdf}}
\hypertarget{link_034}{\includepdf[pages={-}]{WP_pdfs/MP3_034.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_035}{\includepdf[pages={-}]{WP_pdfs/MP3_035.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_036}{\includepdf[pages={-}]{WP_pdfs/MP3_036.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_037}{\includepdf[pages={-}]{WP_pdfs/MP3_037.pdf}}
\hypertarget{link_038}{\includepdf[pages={-}]{WP_pdfs/MP3_038.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_039}{\includepdf[pages={-}]{WP_pdfs/MP3_039.pdf}}
\hypertarget{link_040}{\includepdf[pages={-}]{WP_pdfs/MP3_040.pdf}}
\hypertarget{link_041}{\includepdf[pages={-}]{WP_pdfs/MP3_041.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_042}{\includepdf[pages={-}]{WP_pdfs/MP3_042.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_043}{\includepdf[pages={-}]{WP_pdfs/MP3_043.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_044}{\includepdf[pages={-}]{WP_pdfs/MP3_044.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_045}{\includepdf[pages={-}]{WP_pdfs/MP3_045.pdf}}
\hypertarget{link_046}{\includepdf[pages={-}]{WP_pdfs/MP3_046.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_047}{\includepdf[pages={-}]{WP_pdfs/MP3_047.pdf}}
\hypertarget{link_048}{\includepdf[pages={-}]{WP_pdfs/MP3_048.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_049}{\includepdf[pages={-}]{WP_pdfs/MP3_049.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_050}{\includepdf[pages={-}]{WP_pdfs/MP3_050.pdf}}
\hypertarget{link_051}{\includepdf[pages={-}]{WP_pdfs/MP3_051.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_052}{\includepdf[pages={-}]{WP_pdfs/MP3_052.pdf}}
\hypertarget{link_053}{\includepdf[pages={-}]{WP_pdfs/MP3_053.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_054}{\includepdf[pages={-}]{WP_pdfs/MP3_054.pdf}}
\hypertarget{link_055}{\includepdf[pages={-}]{WP_pdfs/MP3_055.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_056}{\includepdf[pages={-}]{WP_pdfs/MP3_056.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_057}{\includepdf[pages={-}]{WP_pdfs/MP3_057.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_058}{\includepdf[pages={-}]{WP_pdfs/MP3_058.pdf}}
\hypertarget{link_059}{\includepdf[pages={-}]{WP_pdfs/MP3_059.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_060}{\includepdf[pages={-}]{WP_pdfs/MP3_060.pdf}}
\hypertarget{link_061}{\includepdf[pages={-}]{WP_pdfs/MP3_061.pdf}}
\hypertarget{link_062}{\includepdf[pages={-}]{WP_pdfs/MP3_062.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_063}{\includepdf[pages={-}]{WP_pdfs/MP3_063.pdf}}
\hypertarget{link_064}{\includepdf[pages={-}]{WP_pdfs/MP3_064.pdf}}
\hypertarget{link_065}{\includepdf[pages={-}]{WP_pdfs/MP3_065.pdf}}
\hypertarget{link_066}{\includepdf[pages={-}]{WP_pdfs/MP3_066.pdf}}
\hypertarget{link_067}{\includepdf[pages={-}]{WP_pdfs/MP3_067.pdf}}
\hypertarget{link_068}{\includepdf[pages={-}]{WP_pdfs/MP3_068.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_069}{\includepdf[pages={-}]{WP_pdfs/MP3_069.pdf}}
\hypertarget{link_070}{\includepdf[pages={-}]{WP_pdfs/MP3_070.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_071}{\includepdf[pages={-}]{WP_pdfs/MP3_071.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_072}{\includepdf[pages={-}]{WP_pdfs/MP3_072.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_073}{\includepdf[pages={-}]{WP_pdfs/MP3_073.pdf}}
\hypertarget{link_074}{\includepdf[pages={-}]{WP_pdfs/MP3_074.pdf}}
\hypertarget{link_075}{\includepdf[pages={-}]{WP_pdfs/MP3_075.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_076}{\includepdf[pages={-}]{WP_pdfs/MP3_076.pdf}}
\hypertarget{link_077}{\includepdf[pages={-}]{WP_pdfs/MP3_077.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_078}{\includepdf[pages={-}]{WP_pdfs/MP3_078.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_079}{\includepdf[pages={-}]{WP_pdfs/MP3_079.pdf}}
\hypertarget{link_080}{\includepdf[pages={-}]{WP_pdfs/MP3_080.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_081}{\includepdf[pages={-}]{WP_pdfs/MP3_081.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
%\hypertarget{link_082}{\includepdf[pages={-}]{WP_pdfs/MP3_082.pdf}}
\hypertarget{link_083}{\includepdf[pages={-}]{WP_pdfs/MP3_083.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
%\hypertarget{link_084}{\includepdf[pages={-}]{WP_pdfs/MP3_084.pdf}}
\hypertarget{link_085}{\includepdf[pages={-}]{WP_pdfs/MP3_085.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_086}{\includepdf[pages={-}]{WP_pdfs/MP3_086.pdf}}
\hypertarget{link_087}{\includepdf[pages={-}]{WP_pdfs/MP3_087.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_088}{\includepdf[pages={-}]{WP_pdfs/MP3_088.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_089}{\includepdf[pages={-}]{WP_pdfs/MP3_089.pdf}}
\hypertarget{link_090}{\includepdf[pages={-}]{WP_pdfs/MP3_090.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_091}{\includepdf[pages={-}]{WP_pdfs/MP3_091.pdf}}
\hypertarget{link_092}{\includepdf[pages={-}]{WP_pdfs/MP3_092.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_093}{\includepdf[pages={-}]{WP_pdfs/MP3_093.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_094}{\includepdf[pages={-}]{WP_pdfs/MP3_094.pdf}}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\hypertarget{link_095}{\includepdf[pages={-}]{WP_pdfs/MP3_095.pdf}}

\includepdf[pages={-}]{figures/Blank_Page.pdf}
\includepdf[pages={-}]{figures/Blank_Page.pdf}
\includepdf[pages=-]{figures/MP3_Back_Cover_FINAL.pdf}

==> not-yet-mentioned-WPs.tex <==
White Papers not yet mentioned:




%53 (MP3-054)	(PHELIX facility)

%58 (MP3_059)	Nuclear physics research in laser induced plasma with a multi-petawatt laser system: production and decay studies of cosmogenic 26Al

%27 (MP3_028)	MP3 Opportunities for Benchmark-quality Lab-Astro Experiments
%80 (MP3_081)	Understanding Transients: Needs from the Laboratory Astrophysics Community
%20 (MP3_021)	Relativistic Electron Isochoric Heating with Petawatt Femtosecond Lasers for Creation of Warm Dense Matter %This one frankly doesn't really do a good job of saying why MPW is needed



